Zero-Knowledge Location Privacy via Accurate Floating-Point SNARKs

We introduce Zero-Knowledge Location Privacy (ZKLP), enabling users to prove to third parties that they are within a specified geographical region while not disclosing their exact location. ZKLP supports varying levels of granularity, allowing for customization depending on the use case. To realize ZKLP, we introduce the first set of Zero-Knowledge Proof (ZKP) circuits that are fully compliant to the IEEE 754 standard for floating-point arithmetic. Our results demonstrate that our floating point circuits amortize efficiently, requiring only $64$ constraints per multiplication for $2^{15}$ single-precision floating-point multiplications. We utilize our floating point implementation to realize the ZKLP paradigm. In comparison to a baseline, we find that our optimized implementation has $15.9 \times$ less constraints utilizing single precision floating-point values, and $12.2 \times$ less constraints when utilizing double precision floating-point values. We demonstrate the practicability of ZKLP by building a protocol for privacy preserving peer-to-peer proximity testing - Alice can test if she is close to Bob by receiving a single message, without either party revealing any other information about their location. In such a configuration, Bob can create a proof of (non-)proximity in $0.26 s$, whereas Alice can verify her distance to about $470$ peers per second

==> Protocols/circuit_IntOps.tex <==
\begin{figure*}
  \centering
  \footnotesize
    \begin{minipage}{0.28\textwidth}
        \centering
      \begin{minipage}{\textwidth}
          \underline{$\AssertBitLength(\var{v}, L)$, based on bit decomposition}
        % \vspace{-0.1em} 
      \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
        \Require $2^{L} < p$
        \State Receive hint $\{\var{v}_i\}^{L - 1}_{i = 0} = \Computation_{\mathsf{Dec}}(\var{v})$ 
        \For{$i \in [0, L - 1]$}
            \State $\var{v}_i(1 - \var{v}_i) = 0$
        \EndFor
        \State $\var{v} = \sum_{i = 0}^{L - 1}2^i \var{v}_i$
      \end{algorithmic}
      \underline{$\AssertBitLength(\var{v}, L)$, based on lookup argument}
        % \vspace{-0.1em} 
      \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
        \Require $2^{L} < p$
        \State Receive hint $\{\var{v}'_i\}^{L / T - 1}_{i = 0} = \Computation_{\mathsf{Dec}'}(\var{v})$ 
        \For{$i \in [0, L / T - 1]$}
            \State $\mathbf{t}_\mathsf{RC} \coloneqq \mathbf{t}_\mathsf{RC} \cup \var{v}'_i$
        \EndFor
        \State $\var{v} = \sum_{i = 0}^{L/T - 1}2^{iT} \var{v}'_i$
      \end{algorithmic}
      \end{minipage}
      \caption{
      Circuit for checking $\var{v} \in [0, 2^L - 1]$.
      % \jens{Short Note: 1\{P\} checks whether the predicate in the brackets asserts to true. We can state that we set this as constraint, i.e. whenever such a statement fails the system aborts. Makes it a lot more concise so we don't waste lines}
      }
      \label{figure:assert_bit_length}
    \end{minipage}
    \begin{minipage}{0.22\textwidth}
        \centering
      \begin{minipage}{\textwidth}
      \underline{$\CircuitAbs(\var{v}, L)$}
      \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
        \Require $2^L < (p - 1) / 2$
        \State Receive hint $\Computation_{\mathsf{GEZ}}(\var{v}) = \signBitShort$
        \State $\signBitShort(1-\signBitShort)=0$
        % \State Receive hint $\Computation_{\mathsf{GEZ}}(\var{v}) = \signBitShort$ from the prover
        % \State $\AssertIsBool(\signBitShort)$
        % \State $\signBitShort(1-\signBitShort)=0$
        % \State $s \xleftarrow{} \CircuitGreaterThanZero(v)$
        % \State $\var{abs} \coloneqq \Select(\signBitShort, \var{v}, -\var{v})$
        \State $\absoluteValueShort \coloneqq (\signBitShort) \, ? \, \var{v} \, : \, -\var{v}$
        \State $\AssertBitLength(\absoluteValueShort, L)$
        \State \Return $\signBitShort, \absoluteValueShort$
        % \If{\CheckPredicate{$\AssertBitLength(\var{abs}, L)$}}
        % \State \Return $\var{abs}, \var{is\_ge\_0}$
        % \EndIf
        % Add more states as needed
      \end{algorithmic}
      \end{minipage}
      \caption{Circuit for computing sign and absolute value.}
      \label{figure:abs_and_is_positive}
    \end{minipage}\begin{minipage}{0.2\textwidth}
  \begin{minipage}{\textwidth}
    \underline{$\CircuitMax(\var{x}, \var{y}, L)$}
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $2^L < (p - 1) / 2$
    \State $\signBitShort, \_ \coloneqq \CircuitAbs(\var{x} - \var{y}, L)$
    \State \Return $(\signBitShort) \, ? \, \var{x} \, : \, \var{y}$
  \end{algorithmic}
  \underline{$\CircuitMin(\var{x}, \var{y}, L)$}
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $2^L < (p - 1) / 2$
    \State $\signBitShort, \_ \coloneqq \CircuitAbs(\var{x} - \var{y}, L)$
    \State \Return $(\signBitShort) \, ? \, \var{y} \, : \, \var{x}$
  \end{algorithmic}
  \end{minipage}
  \caption{Circuits for computing sign \& absolute value $(\CircuitAbs)$ and maximum $(\CircuitMax)$ \& minimum values $(\CircuitMin)$.}
  \label{figure:combined_circuits}
    \end{minipage}\hfill\begin{minipage}{0.2\textwidth}
  \begin{minipage}{\textwidth}
    \underline{$2^\var{d} = 1 \shl \var{d}$}    % \vspace{-0.1em} 
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $\var{d} \in [0, K], 2^{K} < p$
    \State Receive hint $\var{r} = \Computation_\mathsf{Pow2}(\var{d})$
    \State $\mathbf{t}_\mathsf{Pow2} \coloneqq \mathbf{t}_\mathsf{Pow2} \cup (\var{d}, \var{r})$
    \State \Return $\var{r}$
    % Add more states as needed
  \end{algorithmic}
    \underline{$\var{v} \shl \var{d}$}    % \vspace{-0.1em} 
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $\var{v} \in [0, 2^L - 1]$, $\var{d} \in [0, K]$, $2^{L + K} < p$
    \State \Return $\var{v} \cdot 2^\var{d}$
    % Add more states as needed
  \end{algorithmic}
  \columnbreak
      \underline{$\var{v} \shr \var{d}$}
    % \vspace{-0.1em} 
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $\var{v} \in [0, 2^L - 1]$, $\var{d} \in [0, K]$, $2^{L + K} < p$
    \State $\var{v'} \coloneqq \var{v} \cdot 2^{K - \var{d}}$
    \State Receive hints $\var{q}, \var{r} = \Computation_{\mathsf{Div}}(\var{v}', 2^{K})$ 
    \State $\AssertBitLength(\var{q}, L)$
    \State $\AssertBitLength(\var{r}, K)$
    \State $\var{v}' = \var{q} \cdot 2^K + \var{r}$
    \State \Return $\var{q}$
    % Add more states as needed
  \end{algorithmic}
  \end{minipage}
    \end{minipage}
\end{figure*}

==> Protocols/gadget_Abs.tex <==

\algrenewcommand\alglinenumber[1]{\footnotesize\textbf{#1:}}

% \begin{figure}[t!]
%   \centering
%   \footnotesize
%   \fbox{
%   \begin{minipage}{0.7\columnwidth}
%   \underline{$\AbsAndIsPositive(\var{v}, L)$}
%     % \vspace{-0.1em} 
%   \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
%     \State Receive hint $\var{is\_ge\_0}$ from the prover
%     \State $\AssertIsBool(\var{is\_ge\_0})$
%     \State $\var{abs} \coloneqq \Select(\var{is\_ge\_0}, \var{v}, -\var{v})$
%     \State $\AssertBitLength(\var{abs}, L)$
%     \State \Return $\var{abs}, \var{is\_ge\_0}$
%     % \If{\CheckPredicate{$\AssertBitLength(\var{abs}, L)$}}
%     % \State \Return $\var{abs}, \var{is\_ge\_0}$
%     % \EndIf
%     % Add more states as needed
%   \end{algorithmic}
%   \end{minipage}
%   }
%   \caption{Circuit for computing sign and absolute value}
%   \label{figure:abs_and_is_positive}
% \end{figure}

% \begin{figure}[t!]
%   \centering
%   \footnotesize
%   \fbox{
%   \begin{minipage}{0.7\columnwidth}
%   \underline{$\AbsAndIsPositive(\var{v}, L)$}
%     % \vspace{-0.1em} 
%   \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
%     \State Receive hint $\Computation_{\mathsf{GTZ}}(\var{v}) = \signBitShort$ from the prover
%     % \State $\AssertIsBool(\signBitShort)$
%     \State $\signBitShort(1-\signBitShort)=0$
%     % \State $\var{abs} \coloneqq \Select(\signBitShort, \var{v}, -\var{v})$
%     \State $\absoluteValueShort \coloneqq (\signBitShort) \, ? \, \var{v} \, : \, -\var{v}$
%     \State $\AssertBitLength(\absoluteValueShort, L)$
%     \State \Return $\signBitShort, \absoluteValueShort$
%     % \If{\CheckPredicate{$\AssertBitLength(\var{abs}, L)$}}
%     % \State \Return $\var{abs}, \var{is\_ge\_0}$
%     % \EndIf
%     % Add more states as needed
%   \end{algorithmic}
%   \end{minipage}
%   }
%   \caption{Circuit for computing sign and absolute value\jens{Split into $C_{ABS}$ and $C_{GTZ}$, where $C_{ABS}$ uses $C_{GTZ}$ as sub-circuit? Would clarify figure 4, which would not have to use $C_{ABS}$.}}
%   \label{figure:abs_and_is_positive}
% \end{figure}


\begin{figure}[t!]
  \centering
  \footnotesize
  \fbox{
  \begin{minipage}{0.7\columnwidth}
  \underline{$\CircuitAbs(\var{v}, L)$}
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $2^L < (p - 1) / 2$
    \State Receive hint $\Computation_{\mathsf{GEZ}}(\var{v}) = \signBitShort$ from the prover 
    \State $\signBitShort(1-\signBitShort)=0$
    % \State Receive hint $\Computation_{\mathsf{GEZ}}(\var{v}) = \signBitShort$ from the prover
    % \State $\AssertIsBool(\signBitShort)$
    % \State $\signBitShort(1-\signBitShort)=0$
    % \State $s \xleftarrow{} \CircuitGreaterThanZero(v)$
    % \State $\var{abs} \coloneqq \Select(\signBitShort, \var{v}, -\var{v})$
    \State $\absoluteValueShort \coloneqq (\signBitShort) \, ? \, \var{v} \, : \, -\var{v}$
    \State $\AssertBitLength(\absoluteValueShort, L)$
    \State \Return $\signBitShort, \absoluteValueShort$
    % \If{\CheckPredicate{$\AssertBitLength(\var{abs}, L)$}}
    % \State \Return $\var{abs}, \var{is\_ge\_0}$
    % \EndIf
    % Add more states as needed
  \end{algorithmic}
  \end{minipage}
  }
  \caption{Circuit for computing sign and absolute value.}
  \label{figure:abs_and_is_positive}
\end{figure}


==> Protocols/gadget_Max_Min.tex <==
\algrenewcommand\alglinenumber[1]{\footnotesize\textbf{#1:}}

% \begin{figure}[t!]
%   \centering
%   \footnotesize
%   \fbox{
%   \begin{minipage}{0.7\columnwidth}
%   \underline{$\CircuitMax(\var{x}, \var{y}, L)$}
%     % \vspace{-0.1em} 
%   \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
%     \State $\signBitShort \coloneqq \IsPositive(\var{x} - \var{y}, L)$
%     % \State \Return $\Select(\var{diff\_is\_positive}, \var{x}, \var{y})$
%     \State \Return $(\signBitShort) \, ? \, \var{x} \, : \, \var{y}$
%     % Add more states as needed
%   \end{algorithmic}
%   \underline{$\CircuitMin(\var{x}, \var{y}, L)$}
%     % \vspace{-0.1em} 
%   \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
%     \State $\var{diff\_is\_positive} \coloneqq \IsPositive(\var{x} - \var{y}, L)$
%     \State \Return $\Select(\var{diff\_is\_positive}, \var{y}, \var{x})$
%     % Add more states as needed
%   \end{algorithmic}
%   \end{minipage}
%   }
%   \caption{Circuit for computing maximum and minimum values}
%   \label{figure:max_min}
% \end{figure}


\begin{figure}[t!]
  \centering
  \footnotesize
  \fbox{
  \begin{minipage}{0.4\columnwidth}
  \underline{$\CircuitMax(\var{x}, \var{y}, L)$}
    % \vspace{-0.1em} 
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $2^L < (p - 1) / 2$
    \State $\signBitShort, \_ \coloneqq \CircuitAbs(\var{x} - \var{y}, L)$
    % \State \Return $\Select(\var{diff\_is\_positive}, \var{x}, \var{y})$
    \State \Return $(\signBitShort) \, ? \, \var{x} \, : \, \var{y}$
    % Add more states as needed
  \end{algorithmic}
  \underline{$\CircuitMin(\var{x}, \var{y}, L)$}
    % \vspace{-0.1em} 
  \begin{algorithmic}[1] % The number [1] indicates that lines are numbered
    \Require $2^L < (p - 1) / 2$
    \State $\signBitShort, \_ \coloneqq \CircuitAbs(\var{x} - \var{y}, L)$
    % \State \Return $\Select(\var{diff\_is\_positive}, \var{x}, \var{y})$
    \State \Return $(\signBitShort) \, ? \, \var{y} \, : \, \var{x}$
    % Add more states as needed
  \end{algorithmic}
  \end{minipage}
  }
  \caption{Circuit for maximum \& minimum values.}
  \label{figure:max_min}
\end{figure}


==> Tables/table_test.tex <==

\newcommand{\customarrowLeft}[1]{%
  \makebox[#1]{%
    \hspace*{-4pt}% Adjust this value as needed for alignment
    $\xleftarrow{\hspace*{#1}}$%
    \hspace*{-4pt}% Adjust this value as needed for alignment
  }
}
\newcommand{\customarrowRight}[1]{%
  \makebox[#1]{%
    \hspace*{-4pt}% Adjust this value as needed for alignment
    $\xrightarrow{\hspace*{#1}}$%
    \hspace*{-4pt}% Adjust this value as needed for alignment
  }
}


\begin{figure*}[!ht]
    \raggedright
    \label{fig:mytable} % Label for referencing
    \resizebox{.8\textwidth}{!}{ % Adjust the scale as needed
        \begin{tabularx}{\textwidth}{l*{45}{p{0.2mm}|}}
\cmidrule(l){1-46}
& \multicolumn{45}{c}{\textbf{Resolution}} \\
\cmidrule(l){2-46}
% & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{1} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{2} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{3} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{4} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{5} \customarrowRight{4.2em}} \\
% \cmidrule(l){2-46}
% \textbf{P6}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{P12}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F32}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F64}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% & \multicolumn{9}{c}{\customarrowLeft{3.4em} \textbf{1 ... 6} \customarrowRight{3.4em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{7} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{8} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{9} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{10} \customarrowRight{4.2em}} \\
% \cmidrule(l){2-46}
% \textbf{P6}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{P12}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F32}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F64}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
\cmidrule(l){2-46}
& \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{11} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{12} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{13} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{14} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{15} \customarrowRight{4.2em}} \\
\cmidrule(l){2-46}
\textbf{P6}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} \\
\cmidrule(l){2-46}
\textbf{P12}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
\cmidrule(l){2-46}
\textbf{FP32}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} \\
\cmidrule(l){2-46}
\textbf{FP64}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
\cmidrule(l){2-46}
\end{tabularx}
    }
\caption{Testing proof generation for ZKLP for resolutions $11$ to $15$ for fixed-point (P6, P12), single precision (FP32) and double precision (FP64) floating-point values. For a given resolution, test cases logarithmically approach the boundary of a hexagon. All tests are for Groth16 over BN254. For resolution $1-10$, all tests pass. Green $=$ success, Red $=$ fail.}
% If a cell is green, proof generation succeeds. If a cell is red, proof generation fails.
\label{figure:resolutionComparison}
\end{figure*}


% \begin{table*}[!t]
% \centering
% \caption{Testing $\CircuitZKLP$ for resolutions $1$ to $15$ for fixed-point (P6, P12), single precision (F32) and double precision (F64) floating-point values. For a given resolution, test cases logarithmically approach the boundary of a given hexagon. If a cell is green, proof generation succeeds. If a cell is red, proof generation fails. All tests are executed for Groth16 over curve BN254.}
% \renewcommand{\arraystretch}{0.8}
% \begin{tabularx}{\textwidth}{l*{45}{p{0.2mm}|}}
% \cmidrule(l){1-46}
% & \multicolumn{45}{c}{\textbf{Resolution}} \\
% \cmidrule(l){2-46}
% & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{1} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{2} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{3} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{4} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{5} \customarrowRight{4.2em}} \\
% \cmidrule(l){2-46}
% \textbf{P6}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{P12}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F32}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F64}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{6} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{7} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{8} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{9} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{10} \customarrowRight{4.2em}} \\
% \cmidrule(l){2-46}
% \textbf{P6}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{P12}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F32}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F64}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{11} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{12} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{13} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{14} \customarrowRight{4.2em}} & \multicolumn{9}{c}{\customarrowLeft{4.2em} \textbf{15} \customarrowRight{4.2em}} \\
% \cmidrule(l){2-46}
% \textbf{P6}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} \\
% \cmidrule(l){2-46}
% \textbf{P12}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \textbf{F32}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} \\
% \cmidrule(l){2-46}
% \textbf{F64}  & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} \\
% \cmidrule(l){2-46}
% \end{tabularx}
% \end{table*}
